MobRecon: Mobile-Friendly Hand Mesh Reconstruction from Monocular Image

In this work, we propose a framework for single-view hand mesh reconstruction, which can simultaneously achieve high reconstruction accuracy, fast inference speed, and temporal coherence. Specifically, for 2D encoding, we propose lightweight yet effective stacked structures. Regarding 3D decoding, we provide an efficient graph operator, namely depth-separable spiral convolution. Moreover, we present a novel feature lifting module for bridging the gap between 2D and 3D representations. This module begins with a map-based position regression (MapReg) block to integrate the merits of both heatmap encoding and position regression paradigms for improved 2D accuracy and temporal coherence. Furthermore, MapReg is followed by pose pooling and pose-to-vertex lifting approaches, which transform 2D pose encodings to semantic features of 3D vertices. Overall, our hand reconstruction framework, called MobRecon, comprises affordable computational costs and miniature model size, which reaches a high inference speed of 83FPS on Apple A14 CPU. Extensive experiments on popular datasets such as FreiHAND, RHD, and HO3Dv2 demonstrate that our MobRecon achieves superior performance on reconstruction accuracy and temporal coherence. Our code is publicly available at https://github.com/SeanChenxy/HandMesh.

==> Figures/fig_map_sup.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.9\linewidth]{map_sup.pdf}
\caption{Visualization of heatmap in heatmap+soft-argmax paradigm. The training supervision is the same as our MapReg, i.e., without heatmap loss. The blue points indicate predicted 2D positions.}
\label{fig:mapsup}
\end{center}
\vspace{-0.4cm}
\end{figure}


==> Sections/supplement_in_full.tex <==
\section*{Supplementary Materials}



==> Tables/tab_2dacc_bak.tex <==
\begin{table*}[t]
\small
\renewcommand{\arraystretch}{1.}
\setlength\tabcolsep{2pt}
\centering
\begin{tabular}{c | c c c c c | c c c c c c c}
\hline
\multirow{2}{*}{2D representation}   & \multicolumn{5}{c|}{2D part}  & \multicolumn{7}{c}{2D-to-3D part} \\
& Mult-Adds & \#Param & UVE$\downarrow$ & 2D AUC$\uparrow$ & 2D Acc$\downarrow$ & Pose pooling & Lifting & Mult-Adds & \#Param & PJ$\downarrow$ & 3D AUC$\uparrow$ & 3D Acc $\downarrow$  \\
\hline
$-$   & \multicolumn{5}{c|}{$-$} & Global pooling & FC & 3.2M & 3.2M & 7.55 & 0.850 & 10.12 \\
$\mathbf H_p$ w/o skip.& 57.7M & 1.4M & 6.72 & 0.796 & 2.57 & \multicolumn{7}{c}{$-$} \\
$\mathbf H_p$          & 57.7M & 1.4M & 4.57 & 0.857 & 2.41 & Joint-wise pooling & PVL & 0.4M & 1029 & 7.41 & 0.852 & 9.11 \\
$\mathbf H_p$+soft-argmax      & 57.7M & 1.4M & 4.24 & 0.865 & 2.32 & Grid sampling  & PVL & 0.3M & 1029 & 7.28 & 0.856 & 8.32 \\
$\mathbf L_p$ w/ reg.         & 0.1M & 0.1M & 4.85 & 0.847 & 2.16 & Grid sampling  & PVL & 0.3M & 1029 & 7.11 & 0.859 & 6.14 \\
$\mathbf L_p$ w/ MapReg (ours)& 47.5M & 1.5M & \bf 4.13 & \bf 0.870 & \bf 2.04 & Grid sampling  & PVL & 0.3M & 1029 & \bf 6.95 & \bf 0.862 & \bf 5.41 \\
\hline
\end{tabular}
\caption{Ablation study of feature lifting module. The first line is the setting of CMR \cite{bib:CMR} (the last row of Table~\ref{tab:stack}). ``skip., reg.'' denote skip connection and direct regression. 2D and 3D accuracy are tested on RHD and FreiHAND, respectively. Acc is \textit{w.r.t.} HO3Dv2.}
\label{tab:2d}
\vspace{-0.3cm}
\end{table*}
